Benchmarking LLM-Driven Network Configuration Repair

There is a rapidly growing interest in using Large Language Models (LLMs) to automate complex network operations, but their reliable adoption requires rigorous assessment of their effectiveness and safety. Existing benchmarks do not address whether LLMs can successfully resolve errors in large-scale, interdependent network configurations without introducing new disruptions. Developing such a benchmark is challenging: scenarios must be diverse and increasingly complex, yet their evaluation must be straightforward and meaningful. In this paper, we present Cornetto, the first benchmark to evaluate LLM-driven network configuration repair functionally and at scale. Cornetto features a generation pipeline that synthesizes representative and plausible misconfiguration scenarios, coupled with an evaluation framework that uses formal verification to assess functional correctness of proposed fixes against ground-truth specifications. Using this pipeline, we synthesize a dataset of 231 problems for fixing configurations across varying network topologies (20--754 nodes) and diverse protocols. We evaluate 9 state-of-the-art LLMs and find that while they show promise, they often introduce regressions and their performance degrades at scale. Our results indicate that reliable LLM-powered network automation requires integrating LLMs into iterative workflows guided by formal verification.

==> chapters/tables-removed.tex <==
\begin{table*}[t]
\centering
\small
\caption{Representative features to cover in the generator and the semantic constraints each requires. \textcolor{blue}{Blue} indicates the feature or constraint is \emph{not present in Metha}.}
\label{tab:features}
\begin{tabular}{p{0.18\textwidth} p{0.30\textwidth} p{0.44\textwidth}}
\toprule
\textbf{Feature / Protocol} & \textbf{What it covers} & \textbf{Semantic constraints to enforce} \\
\midrule
BGP neighbor route-maps (in/out) &
Export/import control; policy by prefix/community &
Route-map \emph{exists before attach}; all referenced objects (prefix-/community-/AS-path lists) \emph{exist}; list entries have valid ranges (e.g., \texttt{ge}/\texttt{le}); no dangling names on rename; guard against policy-induced loops (e.g., via tags). \\

BGP next-hop self (iBGP) &
Correct next-hop propagation under RR/edge egress &
Apply on RRs/egress as needed; avoid unintended rewrite on eBGP; ensure IGP reachability to the rewritten next-hop. \\

Community tagging \& matching &
Intent labeling for policy routing &
Communities from valid domains (\texttt{AS:val} or well-known); use additive set when preserving tags; \textcolor{blue}{\textbf{require send-community on both directions when policies depend on tags}}; consistent rename of defs/uses. \\

\textcolor{blue}{ACL apply (interface in/out)} &
Isolation/allow at network edges &
\textcolor{blue}{\textbf{Define before attach; correct direction; stable rule order; terminal permit/deny as per platform; avoid detaching critical ACLs unless intended.}} \\

OSPF interface cost &
Intra-domain path preference &
Bound cost changes; avoid timer/auth mismatches across link ends; verify ECMP/shortest-path deltas match intent. \\

Aggregates at egress (\texttt{aggregate-address} or static$\rightarrow$Null0 + export map) &
Table size control; prevent noisy specifics &
Ensure aggregate covers components; prevent over-aggregation (no blackholes) via export filters; retain specifics where policy requires. \\

Default information originate (IGP/BGP) &
Default export into domains &
Gate with route-map/condition; ensure downstream next-hop reachability; avoid multi-origin oscillation unless intended. \\

\textcolor{blue}{Route Reflection (iBGP)} &
Scale iBGP; change visibility/next-hops &
\textcolor{blue}{\textbf{Assign clients; avoid cluster-ID collisions; ensure send-community; apply next-hop self where needed; optional hybrid mesh+RR phase; no orphaned iBGP speakers.}} \\

\textcolor{blue}{eBGP over loopbacks (multihop)} &
Resilient sessions across fabrics &
\textcolor{blue}{\textbf{Both sides set update-source loopback and ebgp-multihop; IGP reaches loopbacks; TTL security/BFD where supported; avoid underlay dependency cycles.}} \\

\textcolor{blue}{Controlled redistribution (IGP$\leftrightarrow$BGP)} &
Careful route leaking with safety &
\textcolor{blue}{\textbf{Always via route-map; tag to avoid feedback loops; bound side-effects (prefix growth); disallow unintended transitive leaks.}} \\
\midrule
\textbf{Global invariants} & & \\
\midrule
Two-sided link symmetry &
Interfaces, IP/mask, area on both ends &
Create both interfaces; assign the \emph{same} subnet/prefix; special-case /31 addressing; if area assigned, apply to both ends. (Present in Metha.) \\

BGP neighbor role correctness &
eBGP vs iBGP construction &
If AS differs: neighbor on peer \emph{interface IP} (eBGP); else: neighbor on \emph{router-id} (iBGP). (Present in Metha.) \\

\textcolor{blue}{Area 0 connectivity} &
Backbone correctness &
\textcolor{blue}{\textbf{Backbone (area 0) must remain connected; ABR summaries consistent with connectivity.}} \\

Policy object integrity &
Route-map/prefix/comm/as-path objects &
Objects exist before use; value domains valid; names globally unique or consistently renamed. (Partially present in Metha for lists and maps.) \\
\bottomrule
\end{tabular}
\end{table*}




\section{The \textsc{Cornetto} Benchmark}

\subsection{Task Generation Pipeline}

The task at hand is to create interesting scenarios. Each task consists of:

\begin{itemize}
\item A base, "golden" network-wide configuration. 
\item A faulty network-wide configuration. 
\item The observed effects of the misconfiguration on network behaviour
\end{itemize}

The construction of these components must satisfy the following requirements:

\begin{itemize}
    \item The "golden" configuration should sensibly represent a clean enough real-world configuration. We need to balance this with the automated generation nature and the needed flexibility to cover a representative set of features.
    \item The configuration faults should cover a vast array of features and emerging disruptions in network behaviour. Those effects should be \textit{tangible}, i.e. observable with tools such as a verifier.
    \item The effects we observe must suffice in assessing the damage and the complexity of the fault, and it should enable a way to provide a "symptom list" that can point to the problem (but only with information that could be possibly observed in a realistic setting)
\end{itemize}

\textcolor{red}{We may want to frame this in relation to \textit{Metha} and \textit{NetComplete}--- why even do anything at all? Why are these goals not satisfied by either relying on the cisco grammar or a synthesizer?}

\textcolor{red}{One may consider this a problem that is similar but different to \textit{Configuration Synthesis}: Given \textit{no particular intent}, we need to create a collection of configurations that cover many features/mechanisms and "behaviours".}

Based on those goals, we design the task generation pipeline to work as follows [TODO: Construct a nice diagram]: 

\begin{itemize}
\item The input is a Topology and a list (and a \textit{meta}-configuration) of the mechanisms and features that will be enabled in the constructed network.
\item Each mechanism is associated with 1) A set of semantic constraints for its sound application and 2) A set of dependencies for other mechanisms that must be applied 3) A scope (e.g. RR is applied to an AS)
\item Each mechanism is also associated with a library of mutations that changes the network behaviour. It can range from parameter fuzzing to coordinated faults across the network (e.g. skew cost metrics to break ECMP).
\item A model of the network is generated through the meta-configuration and the config files are rendered through a templating engine that ensures syntactic correctness
\item Based on the model of the network and the defined mutation functions, a faulty network configuration is also generated
\item Batfish observes the discrepancy in network behaviour from various aspects. A formulation, various metrics \textcolor{red}{(that need to be defined!!!)} and a description of the symptoms is generated.
\end{itemize}

% in preamble:
% \usepackage{xcolor}
% Blue marks items NOT present in Metha (per code + paper baseline)



\subsection{Ensuring Configuration Plausibility} During the generation of a network-wide configuration, the pipeline applies each feature in a way that
\begin{enumerate}
    \item Respects dependencies on other features, by applying them in an ordered fashion
    \item Respects the semantic constraints that we set for the \textit{sensible} usage of each feature
\end{enumerate}

\subsection{Breaking the Configs}
\paragraph{Defining the Possible Attacks}
\paragraph{Finding the Attack Surface} aaa
\paragraph{Analysis of the Attacks' Effects on Network Behaviour}

\subsection{Dataset Statistics}

\begin{table}[ht]
    \centering
    \caption{Main-dataset summary (mean and max across scenarios)}
    \label{tab:main_dataset_summary}
    \begin{tabular}{llrr}
    \toprule
    \textbf{} & \textbf{Metric} & \textbf{Mean} & \textbf{Max} \\
    \midrule
    Topology      & Nodes (\#)                    & 86.4   & 754  \\
                  & Configuration lines (LoC)                 & 16.1K  & 200.0K \\
                  & Routes               & 4.6K   & 130.4K \\
                  & Data plane predicates           & 12.7K  & 598.0K \\
    \addlinespace
    Fault impact & Lines edited                  & 50.5   & 345  \\
    &   Routers affected & 5.5 & 20 \\
                  & Routes changed                & 568.4  & 9.2K   \\
                  & Predicates changed            & 1.5K   & 38.4K  \\
                  & Forwarding groups changed     & 82.1   & 651.0  \\
    \addlinespace
    Impact (\%)   & LoC\% changed                 & 0.44   & 5.93   \\
                  & Routes\% changed     & 6.34   & 57.3   \\
                  & Predicates\% changed  & 6.82   & 49.8   \\
    \bottomrule
    \end{tabular}
\end{table}

\begin{figure}[ht]
    \centering
    \begin{tikzpicture}
        \pie[
            text=pin, 
            rotate=90, 
            radius=2, 
            color={gray!20, gray!40, gray!60, gray!80, gray!100, black!70, black!50}
        ]{
            47/BGP (360),
            12/OSPF (94),
            11/Addressing (81),
            10/ISIS (79),
            9/ACL (65),
            7/Redist (50),
            4/Static (30)
        }
    \end{tikzpicture}
    \caption{Distribution of faults by protocol}
    \label{fig:fault_pie}
\end{figure}


\begin{itemize}
\item Topology distribution; feature coverage; policy complexity (route-map clauses, ACL terms); LoC changed vs. "effect"/spec change scatter plots.
\end{itemize}

